Effective Model Sparsification by Scheduled Grow-and-Prune Methods

Deep neural networks (DNNs) are effective in solving many real-world problems. Larger DNN models usually exhibit better quality (e.g., accuracy) but their excessive computation results in long inference time. Model sparsification can reduce the computation and memory cost while maintaining model quality. Most existing sparsification algorithms unidirectionally remove weights, while others randomly or greedily explore a small subset of weights in each layer for pruning. The limitations of these algorithms reduce the level of achievable sparsity. In addition, many algorithms still require pre-trained dense models and thus suffer from large memory footprint. In this paper, we propose a novel scheduled grow-and-prune (GaP) methodology without having to pre-train a dense model. It addresses the shortcomings of the previous works by repeatedly growing a subset of layers to dense and then pruning them back to sparse after some training. Experiments show that the models pruned using the proposed methods match or beat the quality of the highly optimized dense models at 80% sparsity on a variety of tasks, such as image classification, objective detection, 3D object part segmentation, and translation. They also outperform other state-of-the-art (SOTA) methods for model sparsification. As an example, a 90% non-uniform sparse ResNet-50 model obtained via GaP achieves 77.9% top-1 accuracy on ImageNet, improving the previous SOTA results by 1.5%. Code available at: https://github.com/boone891214/GaP.

==> tex/ablation.tex <==
\section{Ablation Study}
In this section, we present some ablation study on the proposed GaP methods.


\subsection{Number of partitions for GaP}

The number of partitions in GaP methods play a key role in obtaining better results. As compared in Table~\ref{tab:ablation_rn50_num_part} and Table~\ref{tab:ablation_trans_num_part}, one partition is not sufficient to preserve the best quality. Too many partitions may reduce quality as well (as shown in the model with six partitions in Table~\ref{tab:ablation_trans_num_part}). Empirically, a small number of equal partitions that naturally follow the structures of the models usually perform {well}. For example, ResNet-50 model is composed of four blocks, each sub-samples from the previous block. Thus a four-partition GaP is a natural choice. Transformer model contains an encoder and a decoder, with the decoder twice the number of attention blocks as the encoder. It is naturally divided to three partitions. 

% \textcolor{red}{It is observed from the results of Transformers that $\kappa=3$-partition is  generally better than $\kappa=6$-partition. One may question whether smaller number of partitions leads to better sparse model and in particular, the comparison between $\kappa=1$ and $\kappa > 1$. Table~\ref{tab:ablation_rn50_num_part} and Table~\ref{tab:ablation_trans_num_part} demonstrate this comparison for the uniform sparsity. When $\kappa=1$, the whole model is pruned to the target sparsity and then grown to dense, which is similar to the dense-sparse-dense (DSD)~\cite{han2016dsd}. There are two major differences between the GaP with $\kappa=1$ and DSD. First, the GaP with $\kappa=1$ has multiple grow and prune steps while the DSD only has one. Second, the DSD aims to obtain good dense models and usually uses much less sparsity (around 0.5) while the goal of GaP is the sparse models and we use 0.9 weight sparsity in the experiment.}

% \textcolor{red}{It can be seen from the tables that $\kappa=1$ leads to much inferior sparse models to $\kappa>1$. This result suggests that partitions in the GaP is critical. We conjecture that a moderate number of partitions outperforms $\kappa=1$ since when $\kappa=1$, more weights are pruned than $\kappa>1$ during the pruning phase, which may be too aggressive in searching for a good sparse mask.}


\begin{table*}[ht]
\small
\centering
\caption{The effect of different number of partitions for ResNet-50 models on ImageNet.}
\scalebox{0.93}{
\begin{tabular}{l | cc | cc }
\toprule
Method & Sparsity Ratio & Distribution & Num. Partitions $\kappa$  & Top-1 Acc (\%)        \\ \midrule
\textbf{\emph{C}-GaP}  & 90\% & uniform & 1 &  75.9 \\ 
\textbf{\emph{C}-GaP}  & 90\% & uniform  & 4 &  76.3  \\ 
\bottomrule
\end{tabular}}
\label{tab:ablation_rn50_num_part}
\end{table*}


\begin{table}[h]
\small
\centering
\caption{The effect of different number of partitions for Transformer models on WMT-14 En-De.}
\scalebox{0.93}{
\begin{tabular}{l | cc | cc }
\toprule
Method & Sparsity Ratio & Distribution & Num. Partitions $\kappa$ & SacreBLEU        \\ \midrule
\textbf{\emph{C}-GaP}  & 90\% & uniform & 1 &  26.8 \\ 
%\textbf{\emph{C}-GaP}  & 0.9 & uniform  & 2 &  26.1  \\ 
\textbf{\emph{C}-GaP}  & 90\% & uniform  & 3 &  27.7  \\ 
\textbf{\emph{C}-GaP}  & 90\% & uniform  & 6 &  27.1  \\ 
\bottomrule
\end{tabular}}
\label{tab:ablation_trans_num_part}
\end{table}


\begin{comment}
\subsection{Partition the model in a random manner}

\begin{table}[h]
\small
\centering
\caption{Different partition strategies of ResNet-50 on ImageNet.}
\scalebox{0.93}{
\begin{tabular}{l | cc | cc | c }
\toprule
Method & Sparsity Ratio & Distribution & Num. Partitions & Partition strategy & Top-1 Acc (\%)        \\ \midrule
% &&& (\%)  & FLOPS   &  (\%)  & FLOPS     \\ 
% &&&& ($\times$e9)   &    &  ($\times$e9)    \\ \midrule
\textbf{\emph{C}-GaP}  & 90\% & non-uniform & 4 & Cyclic &  77.9 \\ 
\textbf{\emph{C}-GaP}  & 90\% & non-uniform  & 4 & Random  &  77.8  \\ 
\bottomrule
\end{tabular}}
\label{tab:ablation_rn50_part_strategy}
\end{table}

We also explore a random partition strategy for each step in the {\em C}-GaP for sparse ResNet-50 models. Unlike the cyclic partition where each partition consists of contiguous layers, a random partition  chooses a uniformly random subset of layers to grow in each step of the GaP process. From Table~\ref{tab:ablation_rn50_part_strategy}, we observe that the random partition is slightly worse than the cyclic partition but still much better than all previous solutions in Table~\ref{tab:rn50_irr}. 
\end{comment}




% \textcolor{red}{Add random partition for transformers, and discuss why it is not good. }

\begin{comment}
\textbf{Generalization to other sparse granularity}

We use unstructured sparsity throughout the paper. In this section, we demonstrate that the GaP is also applicable to other coarse-grained sparse granularity such as the block-wise sparsity. The unit for block-wise sparsity in this experiment is $1\times 8$, i.e., if the weight matrix is viewed as many $1\times 8$ blocks, then the sparsity ratio of the matrix is defined as the ratio of {\em all-zero} blocks. It is often believed that the accuracy would be impacted severely when the block size is 8 or greater. Table~\ref{tab:ablation_trans_block} compares the SacreBleu score of sparse Transformers obtained by the 3-partition cyclic {\em C}-GaP and the prune-from-dense method. It can be seen that the GaP has large improvement over prune-from-dense (27.21 vs. 26.21). This further validates the benefits of mask updating brought by the GaP. 

%a $1\times 8$ block of weights is considered as ``sparse'' only if all eight weights are zeros and the first weight in the block needs to 

\begin{table*}[h]
\small
\centering
\caption{Ablation study on different sparse granularity of Transformer on WMT-14 En-De.}
\scalebox{0.93}{
\begin{tabular}{l | cc | cc }
\toprule
Method & Sparsity Ratio & sparse granularity & Num. Partitions $\kappa$ & BLEU        \\ \midrule
% &&& (\%)  & FLOPS   &  (\%)  & FLOPS     \\ 
% &&&& ($\times$e9)   &    &  ($\times$e9)    \\ \midrule
%\textbf{\emph{C}-GaP}  & 0.8 & unstructured & 3 &  27.68 \\ 
prune-from-dense & 80\% & block $1\times 8$ & - & 26.1 \\ \midrule
\textbf{\emph{C}-GaP}  & 80\% & block $1\times 8$  & 3 &  27.2  \\ 
\bottomrule
\end{tabular}}
\label{tab:ablation_trans_block}
\end{table*}



\end{comment}


==> tex/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? 
%   \item Did you include the license to the code and datasets? 
%   \item Did you include the license to the code and datasets? 
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{}. We are not aware any  potential negative societal impacts of this work.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{}. Proof is in the supplementary materials.
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{}. Most papers on the dataset we use (e.g., ImageNet) do not include an error bar as the accuracy is stable.
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{}. We cite the orginial dataset and models.
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}. We use existing dataset and model architectures.
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}. We use public dataset.
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}. We use public dataset.
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

